Training individually fair ML models with Sensitive Subspace Robustness

We consider training machine learning models that are fair in the sense that their performance is invariant under certain sensitive perturbations to the inputs. For example, the performance of a resume screening system should be invariant under changes to the gender and/or ethnicity of the applicant. We formalize this notion of algorithmic fairness as a variant of individual fairness and develop a distributionally robust optimization approach to enforce it during training. We also demonstrate the effectiveness of the approach on two ML tasks that are susceptible to gender and racial biases.

==> YK-macros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> fairnessThruRobustness.tex <==
\section{Fairness through (distributional) robustness}
\label{sec:fairnessThruRobustness}

To motivate our approach, imagine an auditor investigating an ML model for unfairness. The auditor collects a set of audit data and compares the output of the ML model on comparable samples in the audit data. For example, to investigate whether a resume screening system is fair, the auditor may collect a stack of resumes and change the names on the resumes of Caucasian applicants to names more common among the African-American population. If the system performs worse on the edited resumes, then the auditor may conclude the model treats African-American applicants unfairly. Such investigations are known as \textbf{correspondence studies}, and a prominent example is \citeauthor{bertrand2004Are}'s celebrated investigation of racial discrimination in the labor market. In a correspondence study, the investigator looks for inputs that are comparable to the training examples (the edited resumes in the resume screening example) on which the ML model performs poorly. In the rest of this section, we formulate an optimization problem to find such inputs.

\subsection{Fair Wasserstein distances} Recall $\cX$ and $\cY$ are the spaces of inputs and outputs. To keep things simple, we assume that the ML task at hand is a classification task, so $\cY$ is discrete. We also assume that we have a fair metric $d_x$ of the form 
\[
d_x(x_1,x_2)^2 \triangleq \langle x_1 - x_2,\Sigma(x_1 - x_2)\rangle^{\frac12},
\]
where $\Sigma\in\symm_+^{d\times d}$. For example, suppose we are given a set of $K$ ``sensitive'' directions that we wish the metric to ignore; \ie\ $d(x_1,x_2) \ll 1$ for any $x_1$ and $x_2$ such that $x_1 - x_2$ falls in the span of the sensitive directions. These directions may be provided by a domain expert or learned from data (see Section \ref{sec:computationalResults} and Appendix \ref{sec:dataDriveFairMetric}). In this case, we may choose $\Sigma$ as the orthogonal complement projector of onto the span of the sensitive directions. We equip $\cX$ with the fair metric and $\cZ \triangleq \cX\times\cY$ with
\[
d_z((x_1,y_1),(x_2,y_2)) \triangleq d_x(x_1,x_2) + \infty\cdot \ones\{y_1\ne y_2\}.
\]
We consider $d_z^2$ as a transport cost function on $\cZ$. This cost function encodes our intuition of which samples are comparable for the ML task at hand. We equip the space of probability distributions on $\cZ$ with the fair Wasserstein distance
\[\textstyle
W(P,Q) = \inf_{\Pi\in\cC(P,Q)}\int_{\cZ\times\cZ}c(z_1,z_2)d\Pi(z_1,z_2),
\]
where $\cC(P,Q)$ is the set of couplings between $P$ and $Q$. The fair Wasserstein distance inherits our intuition of which samples are comparable through the cost function; \ie\ the fair Wasserstein distance between two probability distributions is small if they are supported on comparable areas of the sample space.
% As we shall see, equipping $M(\cZ)$ with a Wasserstein distance compels the auditor to compare \textit{individual} users instead of groups of users. 


\subsection{Auditing ML models for algorithmic bias}

To investigate whether an ML model performs disparately on comparable samples, the auditor collects a set of audit data $\{(x_i,y_i)\}_{i=1}^n$ and picks a non-negative loss function $\ell:\cZ\times\cH\to\reals_+$ to measure the performance of the ML model. The auditor solves the optimization problem
\begin{equation}\textstyle
\max_{P:W(P,P_n) \le \eps} \textstyle \int_{\cZ}\ell(z,h)dP(z),
\label{eq:auditorsProblem}
\end{equation}
where $h$ is the ML model, $P_n$ is the empirical distribution of the audit data, and $\eps > 0$ is a small tolerance parameter. We interpret $\eps$ as a moving budget that the auditor may expend to discover discrepancies in the performance of the ML model. This budget forces the auditor to avoid moving samples to incomparable areas of the sample space. We emphasize that \eqref{eq:auditorsProblem} detects \emph{aggregate} violations of individual fairness. In other words, although the violations that the auditor's problem detects are individual in nature, the auditor's problem is only able to detect aggregate violations. We summarize the implicit notion of fairness in \eqref{eq:auditorsProblem} in a definition.

\begin{definition}[distributionally robustly fair (DRF)]
An ML model $h:\cX\to\cY$ is $(\eps,\delta)$-distributionally robustly fair (DRF) WRT the fair metric $d_x$ iff
\begin{equation}\textstyle
\max_{P:W(P,P_n) \le \eps} \textstyle \int_{\cZ}\ell(z,h)dP(z) \le \delta.
\label{eq:correspondenceFairness}
\end{equation}
\end{definition}

Although \eqref{eq:auditorsProblem} is an infinite-dimensional optimization problem, it is convex, so it is possible to solve it exactly by appealing to duality. It is known \citep{blanchet2016Quantifying} that the dual of \eqref{eq:auditorsProblem} is 
\begin{equation}
\begin{aligned}
\textstyle\sup_{P:W(P,P_n) \le \eps}\Ex_P\big[\ell(Z,h)\big] = \inf_{\lambda \ge 0}\{\lambda\eps + \Ex_{P_n}\big[\ell_\lambda^c(Z,h)\big]\}, \\
\textstyle\ell_\lambda^c((x_i,y_i),h) \triangleq \sup_{x\in\cX}\ell((x,y_i),\theta) - \lambda d_x(x,x_i).
\end{aligned}
\label{eq:auditorsProblemDual}
\end{equation}
The function $\ell_\lambda^c$ is called the $c$-transform of $\ell$. This is a univariate optimization problem, and it is amenable to stochastic optimization (see Algorithm \ref{alg:DRObjDual}). To optimize \eqref{eq:auditorsProblemDual}, it is imperative that the auditor is able to evaluate $\partial_x\ell((x,y),h)$. 

\begin{algorithm}[H]
\caption{stochastic gradient method for \eqref{eq:auditorsProblemDual}}
\label{alg:DRObjDual}
\begin{algorithmic}[1]
  \Require starting point $\hlambda_1$, step sizes $\alpha_t > 0$
  \Repeat
    \State draw mini-batch $(x_{t_1},y_{t_1}),\dots,(x_{t_B},y_{t_B})\sim P_n$
    \State $x_{t_b}^* \gets \argmax_{x\in\cX}\ell((x,y_{t_b}),h) - \lambda d_x(x_{t_b},x)$, $b\in[B]$
    \State $\hlambda_{t+1} \gets \max\{0,\hlambda_t - \alpha_t(\eps - \frac{1}{B}\sum_{b=1}^Bd_x(x_{t_b},x_{t_b}^*))\}$
  \Until{converged}
\end{algorithmic}
\end{algorithm}

% We recognize \eqref{eq:auditorsProblemDual} as a Lagrangian version of the optimization problem for generating adversarial examples in ML models:
% \begin{subequations}
% \begin{alignat}{2}
% &\max_{\delta_1,\dots,\delta_n} &\quad & \sum_{i=1}^n\ell((x_i + \delta_i,y_i),h) \\
% & \st           & & d_x(x_i + \delta_i,x_i) \le \eps.
% \label{eq:comparabilityConstraint}
% \end{alignat}
% \label{eq:adversarialLoss}
% \end{subequations}
% We note that \eqref{eq:adversarialLoss} enforces the comparability constraint \eqref{eq:comparabilityConstraint} for all samples in the audit data while \eqref{eq:auditorsProblemDual} allows violations of \eqref{eq:comparabilityConstraint} as long as it is satisfied on average. This suggests \eqref{eq:auditorsProblemDual} is a more powerful adversary than \eqref{eq:adversarialLoss}. 

% Let $\hlambda \ge 0$ be an optimal point of \eqref{eq:auditorsProblemDual}. 
It is known that the optimal point of \eqref{eq:auditorsProblem} is the discrete measure $\frac1n\sum_{i=1}^n\delta_{(T_\lambda(x_i),y_i)}$, where $T_\lambda:\cX\to\cX$ is the \textit{unfair map}
\begin{equation}
T_\lambda(x_i) \gets \argmax_{x\in\cX}\ell((x,y_i),h) - \lambda d_x^2(x,x_i).
\label{eq:unfairMap}
\end{equation}
We call $T_\lambda$ an unfair map because it reveals unfairness in the ML model by mapping samples in the audit data to comparable areas of the sample space that the system performs poorly on. We note that $T_\lambda$ may map samples in the audit data to areas of the sample space that are not represented in the audit data, thereby revealing disparate treatment in the ML model not visible in the audit data alone. We emphasize that $T_\lambda$ more than reveals disparate treatment in the ML model; it \textit{localizes} the unfairness to certain areas of the sample space.

We present a simple example to illustrating fairness through robustness (a similar example appeared in \cite{hashimoto2018Fairness}). Consider the binary classification dataset shown in Figure \ref{fig:toy}. There are two subgroups of observations in this dataset, and (sub)group membership is the protected attribute (\eg\ the smaller group contains observations from a minority subgroup). In the figure, the horizontal axis displays (the value of) the protected attribute, while the vertical axis displays the discriminative attribute. In Figure \ref{fig:baseline_decision} we see the decision heatmap of a vanilla logistic regression, which performs poorly on the blue minority subgroup. A tenable fair metric in this instance is a metric that downweights differences in the horizontal direction. Figure \ref{fig:baseline_map} shows that such classifier is unfair with respect to the aforementioned fair metric, i.e. the \textit{unfair map} \eqref{eq:unfairMap} leads to significant loss increase by transporting mass along the horizontal direction with very minor change of the vertical coordinate.

% A fair classifier should learn to be insensitive to minor perturbations according to the fairness metric to satisfy \eqref{eq:equalLoss}. In our toy example this implies a horizontal decision boundary. In Figure \ref{fig:sensr_decision} this is achieved by the algorithm we propose in the next section.
% This is evident in Figure \ref{fig:baseline_map}.

\begin{figure*}[t]\centering
\begin{subfigure}{.32\textwidth}
  \centering
  \captionsetup{justification=centering}
\vspace{-.3in}
\includegraphics[width=\linewidth]{figs/baseline_decision.pdf}
\vspace{-.25in}
\caption{unfair classifier}
\label{fig:baseline_decision}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \captionsetup{justification=centering}
   \vspace{-.3in}
\includegraphics[width=\linewidth]{figs/baseline_map.pdf}
\vspace{-.25in}
\caption{unfair map}
\label{fig:baseline_map}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \captionsetup{justification=centering}
\vspace{-.3in}
\includegraphics[width=\linewidth]{figs/fair_decision.pdf}
\vspace{-.25in}
\caption{classifier from SenSR}
\label{fig:sensr_decision}
\end{subfigure}
\caption{Figure (a) depicts a binary classification dataset in which the minority group shown on the right of the plot is underrepresented. This tilts the logistic regression decision boundary in favor of the majority group on the left. Figure (b) shows the unfair map of the logistic regression decision boundary. It maps samples in the minority group towards the majority group. Figure (c) shows an algorithmically fair classifier that treats the majority and minority groups identically.}
\vspace{-.2in}
\label{fig:toy}
%\vskip -0.2in
\end{figure*}

\paragraph{Comparison with metric fairness} Before moving on to training individually fair ML models, we compare DRF with metric fairness \eqref{eq:metricFairness}. Although we concentrate on the differences between the two definitions here, they are more similar than different: both formalize the intuition that the outputs of a fair ML model should perform similarly on similar inputs. That said, there are two main differences between the two definitions. 

First, instead of requiring the output of the ML model to be similar on all inputs comparable to a training example, we require the output to be similar to the training label. The two definitions have similar implications. Let $(x_i,y_i)$ be a training example and $x_i'$ be an input point such that $d_x(x_i,x_i') \le \eps$. Dwork et al's definition implies 
\begin{equation}
d_y(h(x_i), h(x_i')) \le Ld_x(x_i,x_i') \le \eps L.
\label{eq:DworkImplication}
\end{equation}
On a single training example, we consider a given ML model $h$ fair if $\sup_{x_i':d_x(x_i,x_i') \le \eps} \ell(y_i, h(x_i')) \le \delta$. This implies
\begin{equation}
\ell(h(x_i), h(x_i')) \le \ell(y_i, h(x_i)) + \ell(y_i, h(x_i')) \le 2\delta.
\label{eq:ourImplication}
\end{equation}
Comparing \eqref{eq:DworkImplication} and \eqref{eq:ourImplication}, we see that the two implications are similar, with $\ell$ in \eqref{eq:ourImplication} playing the role of $d_y$ in \eqref{eq:DworkImplication} and $2\delta$ in \eqref{eq:ourImplication} playing the part of $L$ \eqref{eq:DworkImplication}. The main benefit of our definition is it encodes not only (individual) fairness but also accuracy. 

Second, we consider differences between datasets instead of samples by replacing Dwork et al's fair metric on inputs with the Wasserstein distance (on input distributions) induced by the fair metric. The main benefits of this modifications are (i) it is possible to optimize \eqref{eq:auditorsProblem} efficiently, (ii) we can show this modified notion of individual fairness generalizes. 
% The unfortunate side effect is the additional mathematical details.


\subsection{Fair training with Sensitive Subspace Robustness}

% \section{Fair learning with Sensitive Subspace Robustness}
% \label{sec:sensor}
We cast the fair training problem as training supervised learning systems that are robust to sensitive perturbations. We propose solving the minimax problem
\begin{equation}
\inf_{h\in\cH}\sup_{P:W(P,P_n) \le \eps}\Ex_P\big[\ell(Z,h)\big] = \inf_{h\in\cH}\inf_{\lambda\ge 0}\lambda\eps + \Ex_{P_n}\big[\ell_{\lambda}^c(Z,h)\big],
\label{eq:SenSR}
\end{equation}
where $\ell_\lambda^c$ is defined in \eqref{eq:auditorsProblemDual}.
% Although the inner optimization problem is concave, the outer minimization is generally non-convex. 
This is an instance of a distributionally robust optimization (DRO) problem, and it inherits some of the statistical properties of DRO. To see why \eqref{eq:SenSR} encourages individual fairness, recall the loss function is a measure of the performance of the ML model. By assessing the performance of an ML model by its worse-case performance on hypothetical populations of users with perturbed sensitive attributes, minimizing \eqref{eq:SenSR} ensures the system performs well on all such populations. In our toy example, minimizing \eqref{eq:SenSR} implies learning a classifier that is insensitive to perturbations along the horizontal (i.e. sensitive) direction. In Figure \ref{fig:sensr_decision} this is achieved by the algorithm we describe next.
% We see this in Figure \ref{fig:sensr_decision}.

To keep things simple, we assume the hypothesis class is parametrized by $\theta\in\Theta\subset\reals^d$ and replace the minimization with respect to $\cH$ by minimization with respect to $\theta$. In light of the similarities between the DRO objective function and adversarial training, we borrow algorithms for adversarial training \citep{madry2017Deep} to solve \eqref{eq:SenSR} (see Algorithm \ref{alg:SenSR}).

\begin{algorithm}[H]
\caption{Sensitive Subspace Robustness (SenSR)}
\label{alg:SenSR}
\begin{algorithmic}[1]
  \Require starting point $\hat{\theta}_1$, step sizes $\alpha_t,\beta_t > 0$
  \Repeat
  \State sample mini-batch $(x_1,y_1),\ldots,(x_B,y_B)\sim P_n$
  \State $x_{t_b}^* \gets \argmax_{x\in\cX}\ell((x,y_{t_b}),\theta) - \hlambda_td_x(x_{t_b},x)$, $b\in[B]$
  \State $\hlambda_{t+1} \gets \max\{0,\hlambda_t - \alpha_t(\eps - \frac{1}{B}\sum_{b=1}^Bd_x(x_{t_b},x_{t_b}^*))\}$
  % \Comment{skip this step if solving \eqref{eq:lagrangianSenSR}}
  % \State $\hlambda_{t+1} \gets \argmin_{\lambda \ge 0}\lambda\eps + \Ex_{P_n}\big[\ell_{\lambda}^c(Z,\hat{\theta}_t)\big]$
  \State $\hat{\theta}_{t+1} \gets \hat{\theta}_t - \frac{\beta_t}{B}\sum_{b=1}^B\partial_\theta\ell((x_{t_b}^*, y_{t_b}),\hat{\theta}_t)$
  \Until{converged}
\end{algorithmic}
\end{algorithm}

% Algorithm \ref{alg:SenSR} is an instance of a stochastic gradient method, and its convergence properties are well-studied. If $\ell_\lambda^c$ is convex in $\theta$ and its gradient (with respect to $\theta$) is Lipschitz continuous, then the algorithm finds an $\eps$-suboptimal point of \eqref{eq:SenSR} in at most $O(\frac{1}{\eps^2})$ iterations \cite{nemirovski2009Robust}. If $\ell_\lambda^c$ is non-convex in $\theta$, then the algorithm converges to a stationary point of \eqref{eq:SenSR} \cite{ghadimi2013Stochastic}. We summarize the preceding results in a proposition (see Theorem 2 in Sinha et al \cite{sinha2017Certifying} for a similar result).

% \begin{proposition}
% \label{prop:convergence}
% Let $\sigma^2 = \Ex\big[\|\partial_\theta\ell_\lambda^c(Z,\theta) - \partial L_\lambda^c(\theta)\big]\|_2^2\big]$ and $\eps_0 \ge L_\lambda^c(\theta_0) - \inf_{\theta\in\Theta}L_\lambda^c(\theta)$ be an upper bound of the suboptimality of the initial point $\theta_0$. If $\partial\ell_\lambda^c$ is $L$-Lipschitz in $\theta$ and the algorithm takes constant step sizes $\alpha_t = \min\{\frac1L,(\frac{2B\bar{\eps}_0}{L\sigma^2T})^{\frac12}\}$, then 
% \[\textstyle
% \frac1T\sum_{t=1}^T\Ex\big[\|\nabla L_\lambda^c(\theta_t)\|_2^2\big] \le \frac{2L}{T} + (\frac{8\bar{\eps}_0L\sigma^2}{BT})^{\frac12}.
% \]
% If $L_\lambda^c$ is also convex, then
% \[\textstyle
% \frac1T\sum_{t=1}^T\Ex\big[L_\lambda^c(x_t) - \inf_\theta L_\lambda^c(\theta)\big] \le \frac{L\|x_1 - x^*\|_2^2}{T} + \{(\frac{2\bar{\eps}_0}{L})^{\frac12} + (\frac{L\|x_1 - x^*\|_2^2}{2\bar{\eps}_0})^{\frac12}\}\frac{\sigma}{\sqrt{BT}}.
% \]
% \end{proposition}

\paragraph{Related work} Our approach to fair training is an instance of distributionally robust optimization (DRO). In DRO, the usual sample-average approximation of the expected cost function is replaced by $\hL_{\DRO}(\theta) \triangleq \sup_{P\in\cU}\Ex_P\big[\ell(Z,\theta)\big]$, where $\cU$ is a (data dependent) uncertainty set of probability distributions. The uncertainty set may be defined by moment or support constraints \citep{chen2007Robust,delage2010Distributionally,goh2010Distributionally},  $f$-divergences \citep{ben-tal2012Robust,lam2015Quantifying,miyato2015Distributional,namkoong2016Stochastic}, and Wasserstein distances \citep{shafieezadeh-abadeh2015Distributionally,blanchet2016Robust,esfahani2015Datadriven,lee2017Minimax,sinha2017Certifying}. Most similar to our work is \citet{hashimoto2018Fairness}: they show that DRO with a $\chi^2$-neighborhood of the training data prevents representation disparity, i.e. minority groups tend to suffer higher losses because the training algorithm ignores them.
One advantage of picking a Wasserstein uncertainty set is the set depends on the geometry of the sample space. This allows us to encode the correct notion of individual fairness for the ML task at hand in the Wasserstein distance. 

Our approach to fair training is also similar to adversarial training \citep{madry2017Deep}, which hardens ML models against adversarial attacks by minimizing adversarial losses of the form $\sup_{u\in\cU}\ell(z + u,\theta)$, where $\cU$ is a set of allowable perturbations \citep{szegedy2013Intriguing,goodfellow2014Explaining,papernot2015Limitations,carlini2016Evaluating,kurakin2016Adversarial}. Typically, $\cU$ is a scaled $\ell_p$-norm ball: $\cU = \{u:\|u\|_p \le \eps\}$. Most similar to our work is \cite{sinha2017Certifying}: they consider an uncertainty set that is a Wasserstein neighborhood of the training data. 

There are a few papers that consider adversarial approaches to algorithmic fairness. \cite{zhang2018Mitigating} propose an adversarial learning method that enforces equalized odds in which the adversary learns to predict the protected attribute from the output of the classifier. \citet{edwards2015Censoring} propose an adversarial method for learning classifiers that satisfy demographic parity. \citet{madras2018Learning} generalize their method to learn classifiers that satisfy other (group) notions of algorithmic fairness. \cite{garg2019counterfactual} propose to use adversarial logit pairing \citep{kannan2018adversarial} to achieve fairness in text classification using a pre-specified list of counterfactual tokens.
% \yk{cite more ppl?}

==> intro.tex <==
\section{Introduction}

Today, ML models routinely support high-stakes decision-making processes in criminal justice, hiring, and lending, all of which are domains protected by anti-discrimination law. Although ML models appear to eliminate the biases of a human decision maker, they may perpetuate or even exacerbate biases in the training data \citep{barocas2016Big}. Such biases are especially objectionable when it adversely affects underprivileged groups of users \citep{barocas2016Big}.
% Although the most obvious remedy is to remove the biases in the training data, this is impractical in most applications. This leads to the challenge of developing ML models that remain ``fair'' despite biases in the training data.

In response, the scientific community has proposed many mathematical definitions of algorithmic fairness and approaches to ensure ML models satisfy the definitions. Unfortunately, this abundance of definitions, many of which are incompatible \citep{kleinberg2016Inherent,chouldechova2017Fair}, has hindered the adoption of this work by practitioners. There are two types of formal definitions of algorithmic fairness: group fairness and individual fairness. Most recent work on algorithmic fairness considers group fairness because it is more amenable to statistical analysis \citep{ritov2017conditional}. Despite their prevalence, group notions of algorithmic fairness suffer from certain shortcomings. One of the most troubling is there are many scenarios in which an algorithm satisfies group fairness, but its output is blatantly unfair from the point of view of individual users \citep{dwork2011Fairness}. 

In this paper, we consider individual fairness instead of group fairness. Intuitively, an individually fair ML model treats similar users similarly. Formally, an ML model is a map $h:\cX\to\cY$, where $\cX$ and $\cY$ are the input and output spaces. The leading notion of individual fairness is metric fairness \citep{dwork2011Fairness}; it requires
\begin{equation}
d_y(h(x_1),h(x_2)) \le Ld_x(x_1,x_2)\text{ for all }x_1,x_2\in\cX,
\label{eq:metricFairness}
\end{equation}
where $d_x$ and $d_y$ are metrics on the input and output spaces and $L \in \mathbb{R_+}$. The fair metric $d_x$ encodes our intuition of which samples should be treated similarly by the ML model. We emphasize that $d_x(x_1,x_2)$ being small does not imply $x_1$ and $x_2$ are similar in all respects. Even if $d_x(x_1,x_2)$ is small, $x_1$ and $x_2$ may differ in certain problematic ways, e.g. in their protected/sensitive attributes. This is why we refer to pairs of samples $x_1$ and $x_2$ such that $d_x(x_1,x_2)$ is small as \textit{comparable} instead of similar.

% Individual fairness is not only intuitive; it also has a strong legal foundation. In US labor law, \textit{disparate treatment} occurs when the outcome depends on a sensitive attribute (\eg\ race or gender). In disparate treatment cases, aggregate statistics are only relevant if they pertain to the outcome of the \textit{individual} plaintiff \cite{lindemann1983Employment}. Thus disparate treatment is fundamentally an individual notion of unlawful discrimination. By picking a comparability metric that ignores differences in the sensitive attribute, it is possible to formalize disparate treatment as an instance of individual fairness.

Despite its benefits, individual fairness was dismissed as impractical because there is no widely accepted $d_x$ and $d_y$ for many ML tasks. 
% Unfortunately, in application areas where there is disagreement over the choice of $d_x$ and/or $d_y$, this ambiguity negates most of the benefits of a formal definition of fairness.
\citet{dwork2011Fairness} consider randomized ML algorithms, so $h(x)$ is generally a random variable. They suggest probability metrics (\eg\ total variation distance) as $d_y$ and defer the choice of $d_x$ to regulatory bodies or civil rights organizations. In this paper, we consider two data-driven choices of the fair metric: one for problems in which the sensitive attribute is reliably observed, and another for problems in which the sensitive attribute is unobserved (see Appendix \ref{sec:dataDriveFairMetric}).

% In this paper, we describe 
% \begin{enumerate}
% \item a method for learning a fair metric from human supervision: humans generally agree on what is fair and what is unfair for an ML task; disagreements are rare. Instead of being paralyzed by uncertainty in a few cases, we pick $d_x$ by aggregating human opinions. This addresses the pressing issue of disagreement over the choice of $d_x$.
% \item an adversarial approach to training individually fair ML models: we show that individual fairness is a restricted form of robustness: robustness to certain sensitive perturbations to the inputs of an ML model. This connection allows us to leverage recent advances in adversarial training \citep{madry2017Deep} to train individually fair ML models.
% \end{enumerate}
% The rest of the paper is organized into five sections. In Section \ref{sec:fairnessThruRobustness} we develop a method to investigate algorithmic bias/unfairness in ML models. This leads to a training method that trains ML models to pass such investigations. In Section \ref{sec:metricLearning}, we consider the task of learning a fair metric from human supervision. Our algorithmic developments are followed by a theoretical investigation (see Section \ref{sec:theory}) and an empirical study (see Section \ref{sec:theory}) of the efficacy of the proposed approach on two ML tasks.

We propose an adversarial approach to training individually fair ML models. We first show that individual fairness is a restricted form of robustness: robustness to certain sensitive perturbations to the inputs of an ML model. This connection allows us to leverage recent advances in adversarial training \citep{madry2017Deep} to train individually fair ML models. The rest of the paper is organized in four sections. 
In Section \ref{sec:fairnessThruRobustness}, we describe an approach to audit ML models for algorithmic bias, which leads us to consider an approach to training ML models that passes such audits. We justify the approach theoretically (see Section \ref{sec:theory}) and empirically (see Section \ref{sec:computationalResults}).


==> metricLearning.tex <==
\subsection{Learning the fair metric from human supervision}
\label{sec:metricLearning}

The main barrier to wider adoption of individual fairness is disagreement over the fair metric. In this section, we consider the task of learning a fair metric from human supervision. To keep things simple, we focus on learning a generalized Mahalanobis distance
\begin{equation}
d_x(x_1,x_2) = (\varphi(x_1) - \varphi(x_2))^T\hSigma(\varphi(x_1) - \varphi(x_2))^{\frac12},\label{eq:generalizedMahalanobisDistance}
\end{equation}
where $\varphi(x):\cX\to\reals^d$ is a \emph{known} feature map and $\hSigma\in\symm_+^{d\times d}$ is a covariance matrix, from groups of comparable samples. This type of feedback is common in the literature on debiasing learned representations. For example, method of \cite{Bolukbasi2016Man} for removing gender bias in word embeddings relies on sets of words whose embeddings mainly vary in a gender subspace (\eg\ (king, queen)).

Our approach is based on a factor model 
\[
\varphi_i = A_*u_i + B_*v_i + \eps_i,
\]
where $\varphi_i\in\reals^d$ is the learned representation of $x_i$, $u_i\in\reals^K$ (resp.\ $v_i\in\reals^L$) is the sensitive/irrelevant (resp.\ relevant) attributes of $x_i$ to the task at hand, and $\eps_i$ is an error term. For example, in \cite{Bolukbasi2016Man}, the learned representations are the embeddings of words in the vocabulary, and the sensitive attribute is the gender bias of the words. The sensitive and relevant attributes are generally unobserved.

Recall our goal is to obtain $\hSigma$ so that \eqref{eq:generalizedMahalanobisDistance} is small whenever $v_1\approx v_2$. One possible choice of $\hSigma$ is the projection matrix onto the orthogonal complement of $\ran(A)$. Indeed,
% \[
% d_x(x_1,x_2)^2 = (\varphi_1 - \varphi_2)^T(I - P_{\ran(A)})(\varphi_1 - \varphi_2) \approx (v_1 - v_2)^TB_*^T(I - P_{\ran(A)})B_*(v_1 - v_2),
% \]

\begin{align}
d_x(x_1,x_2)^2 &= (\varphi_1 - \varphi_2)^T(I - P_{\ran(A)})(\varphi_1 - \varphi_2) \label{eq:fair_metric} \\
& \approx (v_1 - v_2)^TB_*^T(I - P_{\ran(A)})B_*(v_1 - v_2),
\end{align}
which is small whenever $v_1\approx v_2$. Although $\ran(A)$ is unknown, it is possible to estimate it from the learned representations and groups of comparable samples by factor analysis. 

The factor model attributes variation in the learned representations to variation in the sensitive and relevant attributes. We consider two samples comparable if their relevant attributes are similar. In other words, if $\cI\subset[n]$ is (the indices of) a group of comparable samples, then
\begin{equation}
H\Phi_{\cI} = HU_{\cI}A_*^T  + \cancelto{\approx 0}{HV_{\cI}B_*^T} + HE_{\cI} \approx HU_{\cI}A_*^T + HE_{\cI},
\label{eq:centersubGroup}
\end{equation}
where $H =I_{\abs{\cI}} - \frac{1}{\abs{\cI}}1_{\abs{\cI}}1_{\abs{\cI}}^T$ is the centering or de-meaning matrix and the rows of $\Phi_{\cI}$ (resp.\ $U_{\cI}$, $V_{\cI}$) are $\varphi_i$ (resp.\ $u_i$, $v_i$). If this group of samples have identical relevant attributes, \ie\ $V_{\cI} = 1_{\abs{\cI}}v^T$ for some $v$, then $HV_{\cI}$ vanishes exactly. As long as $u_i$ and $\eps_i$ are uncorrelated (\eg\ $\Ex\big[u_i\eps_i^T\big] = 0$), \eqref{eq:centersubGroup} implies 
\[
\Ex\big[\Phi_{\cI}^TH\Phi_{\cI}\big] \approx A\Ex\big[U_{\cI}^THU_{\cI}\big]A^T + \Ex\big[E_{\cI}^THE_{\cI}\big],
\] 
This suggests estimating $\ran(A)$ from the learned representations and groups of comparable samples by factor analysis. We summarize our approach in Algorithm \ref{alg:1.1}.

\begin{algorithm}[H]
\caption{estimating $\hSigma$ for the fair metric}
\label{alg:1.1}
\begin{algorithmic}[1]
  \State {\bf Input:} $\{\varphi_i\}_{i=1}^n$, comparable groups $\cI_1,\dots,\cI_G$
  \State $\hA^T \in \argmin_{W_g,A}\{{\textstyle\frac12\sum_{g=1}^G\|H_g\Phi_{\cI_g} - W_gA^T\|_F^2}\}$
  \Comment{factor analysis}
  \State $Q \gets \texttt{qr}(\hA)$ 
  \Comment{get orthonormal basis of $\ran(\hA)$}
  \State $\hSigma \gets I_d - QQ^T$
\end{algorithmic}
\end{algorithm}
